Improved Differentially Private and Lazy Online Convex Optimization

We study the task of $(\epsilon, \delta)$-differentially private online convex optimization (OCO). In the online setting, the release of each distinct decision or iterate carries with it the potential for privacy loss. This problem has a long history of research starting with Jain et al. [2012] and the best known results for the regime of {\epsilon} not being very small are presented in Agarwal et al. [2023]. In this paper we improve upon the results of Agarwal et al. [2023] in terms of the dimension factors as well as removing the requirement of smoothness. Our results are now the best known rates for DP-OCO in this regime. Our algorithms builds upon the work of [Asi et al., 2023] which introduced the idea of explicitly limiting the number of switches via rejection sampling. The main innovation in our algorithm is the use of sampling from a strongly log-concave density which allows us to trade-off the dimension factors better leading to improved results.

==> experiments.tex <==
\section{Experiments}

==> notes.tex <==

\section{Approach based on FTRL+Noise+Coupled Sampling}

Define at every time step $p_t \defeq \argmin_{x \in \K} \sum_{\tau = 1}^{t-1} f_{\tau}(x) + \frac{1}{\eta}R(x) + z_t^{\top}x$ where $z_t \sim \N(0,\sigma I)$

Algorithm is as follows -- 

\begin{algorithm}
        \begin{algorithmic}
        \STATE \textbf{Parameters}: $\sigma, \eta > 0, p \in [0,1]$.
\FOR {$t = 1 \ldots T$}
    \STATE Sample a Bernoulli random variable $Z_t$ with probability $p$.
    \IF {$Z_t = 1$}
    \STATE Sample $z_t \sim \N(0, \sigma \cdot I) $.
    \STATE Output $x_t = \argmin_{x \in \K} \left(\sum_{\tau = 1}^{t-1} l_{\tau}(x) + \frac{1}{\eta}R(x) + z_t^{\top}x\right)$.
    \ELSE
    \STATE Compute probability ratio 
    \[ \frac{\P_{t-1}(x_t)}{\P_t(x_t)}\]
    \ENDIF
    \ENDFOR
\end{algorithmic}
\end{algorithm}


\begin{itemize}
    \item Define at every time step $p_t \defeq \argmin_{x \in \K} \sum_{\tau = 1}^{t-1} f_{\tau}(x) + \frac{1}{\eta}R(x) + z_t^{\top}x$ where $z_t \sim \N(0,\sigma I)$
    \item At every step we will play a point that marginally satisfis $x_t \sim p_t$. However the point will be sampled in a coupled fashion between $p_t$ and $p_{t-1}$. 
    \item \textbf{Regret Analysis}: Since marginally $x_t$ is sampled from $p_t$ we can assume for expected regret analysis that $z_t = z$ for all $t$. At that point we can absorb the noise in the regularizer -- the stability term does not change and the bias term adds another at most $\sigma$ sized term. 
    % \item \textbf{Analyzing Switching}: Like in Tomer's paper we can assume unique minima. If we want to use Tomer's technique we need to bound the total variation distance between successive $p_t$ and $p_{t-1}$. As per Tomer's analysis the expected number of switches = $\sum_{t} TV(p_t, p_{t-1})$. 
    % To bound the total variation distance we note the following property. Consider any time $t$ and any vector $v$ and define 
    % \[ x_t(v) = \argmin_{x \in \K} \sum_{\tau = 1}^{t-1} f_{\tau}(x) + \frac{1}{\eta}R(x) + v\]
    % For any $v$ and I claim that $x_t(v) \in x_{t+1}(v - \nabla f_t(x_t(v)))$. This follows via KKT conditions as the change in v has ensured that the gradient at point $x$ has not changed in both situations. 
    % Therefore we get that $x$ 
    \item \textbf{Analyzing Switching}: To sample in a coupled fashion we use a Metropolis Hastings sampler, i.e. given two distributions $p,q$ and a sample from $p$ we use the following procedure. Evaluate $q(x)/p(x)$. Toss a coin with probability $q(x)/p(x)$, if heads output $x$ otherwise draw a fresh sample from $q$. Following is a proof that the new sample is generated from the distribution $q(x)$. Let new sample be $z$, (proof is for discrete distributions but can be made rigorous with densities)
     \[\Pr(z=x) = \sum_{y} \left( \frac{q(y)}{p(y)} I(y=x) p(y) + \left(1 - \frac{q(y)}{p(y)}\right)q(x)p(y) \right) = q(x)\]
    
    Now it is clear that given any $x \sim p$, the probability of switching when coupling distributions in this way is atmost
    
    \[ ( 1 - q(x)/p(x)) \]
    
    
    
    
    
    Like in Tomer's paper we can assume unique minima. Consider any time $t$ and any vector $v$ and define 
    \[ x_t(v) = \argmin_{x \in \K} \sum_{\tau = 1}^{t-1} f_{\tau}(x) + \frac{1}{\eta}R(x) + v\]
    For any $t, v$ and I claim that $x_t(v) = x_{t+1}(v - \nabla f_t(x_t(v)))$. This follows via KKT conditions as the change in $v$ has ensured that the gradient at point $x$ has not changed in both situations. Define $g_t(v) = v - \nabla f_t(x_t(v))$.
    Therefore we get that for any $x$
    
    \[ \frac{Pr(x_{t+1} = x)}{Pr(x_t = x)} = \frac{\int_{v} I(x_{t+1}(v) = x) \mu(v) dv}{\int_{v} I(x_{t}(v) = x) \mu(v) dv} = \frac{\int_{v} I(x_{t+1}(v) = x) \mu(v) dv}{\int_{v} I(x_{t+1}(g_t(v)) = x) \mu(v) dv} = \frac{\int_{v} I(x_{t+1}(v) = x) \mu(v) dv}{\int_{v} I(x_{t+1}(g_t(v)) = x) \mu(g_t(v)) \left(\frac{\mu(v)}{\mu(g_t(v))}\right) dv}\]
    
    Therefore if we want to show $\frac{Pr(x_{t+1} = x)}{Pr(x_t = x)} \geq c$ it is sufficient to show $\left(\frac{\mu(g_t(v))}{\mu(v)}\right) \leq c$ for all $v$. We wont be able to show it for all $v$ but will be able to show it for all small enough $v$. 
    
    \[ \frac{\mu(g_t(v))}{\mu(v)} = exp \left( \frac{v^2 - (v - \nabla f_t(x_t(v)))^2}{2\sigma^2} \right) = exp \left( \frac{2v^{\top}\nabla f_t(x_t(v)) - \|\nabla f_t(x_t(v)))\|^2}{2\sigma^2} \right)\]
    
    Applying the analysis of the Gaussian mechanism for any $\epsilon \leq 1$ we can show that the above is less than $e^{\epsilon} \leq 1 + \epsilon + \epsilon^2 \leq 1 + 2\epsilon$ if we set $\sigma = O(\frac{\|f_t(x_t(v))\|}{\epsilon}) \leq O(\frac{L}{\epsilon})$. This will require us to remove large values of $v$ (like the $delta$ in Gaussian Mech). We can run the entire analysis conditioned on the event that all sampled $v$ are $<< \sigma \log T$ in norm. This will only cost us $log T$ in regret.
    
    Therefore total expected number of switches are at most $O(T/\epsilon) = O(T/\sigma) = S$. Further for regret we have that upto $O()$
    \[ \text{Regret} = \eta + T/\eta + \sigma\]
    We can set $\sigma = O(T/S)$ and get the regret rate $O(\sqrt{T} + T/S)$.


    \item \textbf{Handwavy extension to DP} -- Basically everytime you switch you suffer a privacy loss. Privacy loss is roughly $1/\sigma$.  This is because since function is bounded total change is bounded and it is to be covered by noise of scale $\sigma$. So total amount of privacy loss with strong comp. $1/\sigma \sqrt{numswtiches} = \sqrt{T}/\sigma^{3/2}$ to get this to be less than $\epsilon$ we need $\sigma = \frac{T^{1/3}}{\epsilon^{2/3}}$. This will get you a total regret of 
        \[\sqrt{T} + \frac{T^{1/3}}{\epsilon^{2/3}}\]
    On the face of it this is better than Kunal's result but to be correct on privacy you have to add a backdoor fixed prob of switching and I guess this will all lead to the same bound as in Kunal's paper. 
\end{itemize}




\section{Explanation of why the tree mechanism works for 1 dimensional abs value and fails for high dimensional convex}

To understand this let me first present an alternate long proof of the tree mechanism for the linear case. I will only present it for T = 3 as the main idea is captured. 

The setup is adversary produces vectors $v_1, v_2, v_3$ and the player produces the following sequence where $z_i$ are all iid noise vectors
\[ x_1 = v_1 + z_1\]
\[ x_2 = v_1 + v_2 + z_2 \]
\[ x_3 = v_1 + v_2 + v_3 + z_2 + z_3\]

Imagine we have a different dataset where $v_1$ is replaced by $v_1'$. Let the players outputs for this be $x_1', x_2', x_3'$. In differential privacy we finally care about the following ratio for any sequence of vectors $a_1, a_2, a_3$

\[\frac{Pr(x_1=a_1,x_2=a_2,x_3=a_3)}{Pr(x'_1=a_1,x'_2=a_2,x'_3=a_3)}\]

Suppose we know that $\|v_1 - v_1'\| \leq 1$, then choosing $z's$ from a distribution $N(0, \frac{1}{\epsilon}I)$ and doing a weak union bound (i.e. composition in privacy terms) will give us

\[\frac{Pr(x_1=a_1,x_2=a_2,x_3=a_3)}{Pr(x'_1=a_1,x'_2=a_2,x'_3=a_3)} \leq e^{3\epsilon}\]

This is the loose analysis which loses 3. The tight analysis will show that this is actually $e^{2\epsilon}$ and this is the crux of tree aggregation. I show that below.

\begin{align*}
    \frac{Pr(x_1=a_1,x_2=a_2,x_3=a_3)}{Pr(x'_1=a_1,x'_2=a_2,x'_3=a_3)} = \frac{Pr(x_1=a_1)}{Pr(x_1'=a_1)} \cdot \frac{Pr(x_2=a_2 | x_1=a_1)}{Pr(x_2'=a_2 | x_1'=a_1)} \cdot \frac{Pr(x_3=a_3 | x_1=a_1, x_2=a_2)}{Pr(x_3'=a_3 | x_2'=a_2, x_1'=a_1)}
\end{align*}

Using the definitions of $x$ and $x'$ and exactly mapping the events above exactly term by term we get the following

\[\frac{Pr(x_1=a_1)}{Pr(x'_1=a_1)} = \frac{Pr(z_1=a_1-v_1)}{Pr(z_1=a_1 - v_1')} \leq e^{\epsilon}\]
\[  \frac{Pr(x_2=a_2 | x_1=a_1)}{Pr(x_2'=a_2 | x_1'=a_1)}  = \frac{Pr(z_2 = a_2 - v_1 - v_2 | z_1=a_1-v_1)}{Pr(z_2 = a_2 - v_1' - v_2 | z_1=a_1 - v_1')} \leq e^{\epsilon}\]
While the above terms are what you imagine, the third term is the winner
\begin{align*}
    \frac{Pr(x_3=a_3 | x_1=a_1, x_2=a_2)}{Pr(x_3'=a_3 | x_2'=a_2, x_1'=a_1)} &= \frac{Pr( z_3 = a_3 - v_1 - v_2 - v_3 - z_2 | z_2 = a_2 - v_1 - v_2, z_1=a_1-v_1)}{Pr(z_3 = a_3 - v_1' - v_2 - v_3 - z_2 | z_2 = a_2 - v_1' - v_2 , z_1=a_1 - v_1')} \\
    &= \frac{Pr( z_3 = a_3 - v_3 - a_2)}{Pr(z_3 = a_3 - v_3 - a_2 )} = 1
\end{align*}

Basically the effect of $v_1$'s change has already been absorbed in the conditioning and therefore does not appear. 

\textbf{SK note:} another simple way of seeing this argument is the following: $x_2$ is independent of $x_1$, and $x_3 = x_2 + v_3 + z_3$.

\paragraph{One dimensional Abs functions with tree agg - Argument}

Again lets consider $T=3$. The setup here is that the adversary at every step plays the function $f_t(x) = |x-v_t|$. We play 


But this also shows why the argument fails for high dimensional convex just fixing the minimizer of $f_1 + z_1$, i.e. conditioning on that does not fix all the values $f_1 + z_1$ as a function and this is what happens in the linear case. 

\section{Hessian analysis}

Let $\ell \in \mathbb{R}^n$ be a given vector. Define the function $\sigma: \mathbb{R}^d \to \mathbb{R}^d$ to be the softmax function defined as:
\[\sigma(z)_i = \frac{\exp(z_i + \ell_i)}{\sum_{j} \exp(z_j + \ell_i)}.\]
\begin{lemma}
Let $Z \sim \mathcal{N}(0, I)$. Then
\[\|\mathbb{E}[\sigma(Z)] - \sigma(0)\|_1 \leq \frac{1}{4}.\]
\end{lemma}
\begin{proof}
\textbf{(This proof is a bit imprecise in the use of the remainder theorem.)}
We have
\[\sigma(Z)_1 - \sigma(0)_1 \approx \nabla \sigma(0)_1 \cdot Z + \frac{1}{2} \nabla^2 \sigma(0)_1 \bullet ZZ^\top.\]
Taking expectations on both sides, we get
\[\mathbb{E}(\sigma(Z)_1) - \sigma(0)_1 \approx \frac{1}{2}\text{Tr}(\nabla^2 \sigma(0)_1),\]
since $\mathbb{E}(Z) = 0$ and $\mathbb{E}(ZZ^\top) = I$. 

Now, for notational convenience, let $\varsigma := \sigma(0)$.
Then, by direct calculation, we have
\[\frac{\partial^2}{\partial z_1^2} \sigma(0)_1 = (\varsigma_1^2-\varsigma_1)(2\varsigma_1 - 1),\]
and for $i > 1$,
\[\frac{\partial^2}{\partial z_i^2} \sigma(0)_1 =  \varsigma_1\varsigma_i(2\varsigma_i - 1).\]
Thus, 
\[\text{Tr}(\nabla^2 \sigma(0)_1) = 2\varsigma_1^2(\textstyle\sum_i \varsigma_i^2 - 1).\]
Hence,
\[|\mathbb{E}[\sigma(Z)_1] - \sigma(0)_1| \approx 2\varsigma_1^2(1-\textstyle\sum_i \varsigma_i^2),\]
and so
\[\|\mathbb{E}[\sigma(Z)] - \sigma(0)\|_1 \approx ({\textstyle\sum}_i 2\varsigma_i^2)(1-{\textstyle\sum}_i \varsigma_i^2) \leq \frac{1}{2}.\]
The last inequality follows because the maximum value of $2x(1-x)$ is $\frac{1}{2}$.
\end{proof}

\textbf{More rigorous analysis follows.}
\begin{lemma}
Let $Z \sim \mathcal{N}(0, I)$. Then we have
\[\|\mathbb{E}[\sigma(Z)] - \sigma(0)\|_1 = O(\log d).\]
\end{lemma}
\begin{proof}
We have
\[\sigma(Z)_1 - \sigma(0)_1 = \nabla \sigma(0)_1 \cdot Z + \frac{1}{2} \nabla^2 \sigma(\xi)_1 \bullet ZZ^\top,\]
where $\xi$ is a point on the line segment joining $0$ to $Z$. Note that this is a function of $Z$ and is hence a random variable itself.
Taking expectations on both sides, we get
\[\mathbb{E}(\sigma(Z)_1) - \sigma(0)_1 = \frac{1}{2}\mathbb{E}(\nabla^2 \sigma(\xi)_1 \bullet ZZ^\top),\]
since $\mathbb{E}(Z) = 0$. 

Now, for notational convenience, let $\varsigma := \sigma(\xi)$.
Then, by direct calculation \textbf{(Please check!)}, we have
\[\nabla^2 \sigma(\xi)_1 = \varsigma_1(e_1e_1^\top - e_1\varsigma^\top - \varsigma e_1^\top - \text{diag}(\varsigma) + 2 \varsigma\varsigma^\top).\]
Now, since $Z \sim \mathcal{N}(0, I)$, whp, for some $c = O(\sqrt{\log d})$, we have $|Z_i| \leq c$ for all $i \in [d]$. Thus, $\|\overrightarrow{ZZ^\top}\|_\infty \leq c^2$, where for a matrix $A$, $\overrightarrow{A}$ denotes the vectorization of matrix $A$. Thus, to bound $\frac{1}{2}\mathbb{E}(\nabla^2 \sigma(\xi)_1 \bullet ZZ^\top)$, we just need to bound the $\|\overrightarrow{\nabla^2 \sigma(\xi)_1}\|_1$. But from the formula above, it is easy to see that $\|\overrightarrow{\nabla^2 \sigma(\xi)_1}\|_1 \leq 6\varsigma_1$. Thus, whp, 
\[\frac{1}{2} \nabla^2 \sigma(\xi)_1 \bullet ZZ^\top \leq 3\varsigma_1 c^2.\]
Summing up similar bounds for $\frac{1}{2} \nabla^2 \sigma(\xi)_i \bullet ZZ^\top$ for $i \in [d]$, and noting that $\sum_i \varsigma_i = 1$, we get the stated bound in the lemma.
\end{proof}



\section{1-D analysis}

We assume here that our loss functions $\ell_t: [0, 1] \to [0, 1]$ are convex and $1$-Lipschitz. Given $\alpha \in (0, 1)$, consider the feature mapping $\Phi: [0, 1] \to \mathbb{R}^D$ where $D = \frac{1}{\alpha}+2$ as follows:
\[\Phi(x) = [1, x, \max\{x, \alpha\}, \max\{x, 2\alpha\}, \ldots, \max\{x, 1\}]^\top.\]
\begin{lemma}
For any convex, 1-Lipschitz function $\ell: [0, 1] \to [0, 1]$, there exists a vector $\tilde{\ell} \in \mathbb{R}^D$ such that for any $x \in [0, 1]$, we have
\[|\ell(x) - \tilde{\ell} \cdot \Phi(x)| \leq 2\alpha.\]
Furthermore, $\|\tilde{\ell}\|_1 \leq 4$.
\end{lemma}
\begin{proof}
\newcommand{\stair}{\texttt{stair}}
\newcommand{\ind}{\mathbb{I}}
Since $\ell$ is convex and $1$-Lipschitz, its derivative $\ell'$ (here, we use the right derivative at any non-differentiable point) is an increasing function mapping $[0, 1]$ to $[-1, 1]$.
Consider the following function $\stair: [0, 1] \to [-1, 1]$:
\[\stair(x) = \ell'(0) + \sum_{i=1}^{1/\alpha} [\ell'(\alpha i) - \ell'(\alpha (i-1))] \cdot \ind[x \geq \alpha i] = \ell'(\alpha \lfloor \tfrac{x}{\alpha}\rfloor).\]
Note that $\stair(x) \leq \ell'(x)$ for all $x \in [0, 1]$. Furthermore, for any $x \in [\alpha i, \alpha (i+1))$, since $\ell'$ is an increasing function, we have $ \ell'(x) - \stair(x) \leq \ell'(\alpha (i+1)) - \ell'(\alpha i)$. Thus, for any $x \in [0, 1]$ we have
\begin{align*}
\left| \int_{u=0}^x \ell'(u)du - \int_{u=0}^x \stair(u)du\right| &\leq \int_{u=0}^1 (\ell'(u) - \stair(u))du \\
&= \sum_{i=0}^{\frac{1}{\alpha}-1} \int_{u=\alpha i}^{\alpha(i+1)}  (\ell'(u) - \stair(u))du \\
&\leq \sum_{i=0}^{\frac{1}{\alpha}-1} \int_{u=\alpha i}^{\alpha(i+1)} (\ell'(\alpha (i+1)) - \ell'(\alpha i))du \\
&= \sum_{i=0}^{\frac{1}{\alpha}-1} (\ell'(\alpha (i+1)) - \ell'(\alpha i))\cdot \alpha \\
&= (\ell'(1) - \ell'(0))\cdot \alpha \\
&\leq 2\alpha.
\end{align*}
Now, note that
\[ \int_{u=0}^x \ell'(u)du = \ell(x) - \ell(0)\]
and
\[\int_{u=0}^x \stair(u)du = \ell'(0)x + \sum_{i=1}^{1/\alpha} [\ell'(\alpha i) - \ell'(\alpha (i-1))] \max\{x, \alpha i\}.\]
Consider the vector $\tilde{\ell} \in \mathbb{R}^D$ defined as
\[\tilde{\ell} = [\ell(0), \ell'(0), [\ell'(\alpha) - \ell'(0)], [\ell'(2\alpha) - \ell'(\alpha)], \ldots, [\ell'(1) - \ell'(1-\alpha)]]^\top.\]
The above observations imply that for all $x \in [0, 1]$, we have
\[\left| \ell(x) -  \tilde{\ell} \cdot \Phi(x)\right| \leq 2\alpha.\]
Furthermore, we have
\[\|\tilde{\ell}\|_1 = \ell(0) + |\ell'(0)| + [\ell'(1) - \ell'(0)] \leq 4.\]
\end{proof}

\subsection{DP 1-D OCO algorithm}

\textcolor{red}{\textbf{Satyen's note: This analysis is incorrect even though the bound it claims is the right one!! Maybe it can be salvaged?}}

In each iteration $t$, replace $\ell_t$ by the linear function $x \mapsto \tilde{\ell}_t \cdot \Phi(x)$ and run the [AS17] algorithm on these linear functions. The algorithm is $(\epsilon, \delta)$-DP with (average) regret bound
\[\frac{1}{\sqrt{T}} + \frac{\sqrt{D \log(1/\delta)}}{\epsilon T}\]
against the linear functions. Since the linear functions approximate the $\ell_t$ functions pointwise with error at most $2\alpha$, the regret against the original $\ell_t$ functions is (up to constant factors)
\[\frac{1}{\sqrt{T}} + \frac{\sqrt{(1/\alpha)\log(1/\delta)}}{\epsilon T} + \alpha.\]
The optimal value of $\alpha$ is $\frac{\log^{1/3}(1/\delta)}{(\epsilon T)^{2/3}}$ leading to a final bound of
\[\frac{1}{\sqrt{T}} + \frac{\log^{1/3}(1/\delta)}{(\epsilon T)^{2/3}}.\]

\subsubsection{Implementation}

To implement the algorithm we would need to solve optimization problem of the following type:
\[\min_{x \in [0, 1]} \sum_{s=1}^{t-1} \tilde{\ell}_t \cdot \Phi(x) + b_t \cdot \Phi(x),\]
where $b_t$ is the noise vector. In general this may not be a convex optimization problem if the coordinates of $\sum_{s=1}^{t-1}\tilde{\ell}_t + b_t$ are negative: specifically, we need the coordinates $2, 3, \ldots, D$ to non-negative to give a convex optimization problem. However I believe we can truncate negative coordinates to $0$ without any issue: this is post-processing so still DP, and I believe the regret bound should remain the same.

\section{Introduction}
\label{sec:intro}

In this paper, we revisit differentially private online convex optimization and resolve remaining open questions in the area. 


\subsection{Setup}
Let $\X \in \reals^d$ and let $D = \max_{x \in X}\|x\|_2$.

\paragraph{Stochastic OCO} In this setup we assume that there exists a distribution $\D$ supported over a subset of convex functions $\F \subseteq \{f:\X \rightarrow \reals | f \text{ is convex}\}$. We assume that for all $f \in \F$ we have that $f$ is $L$-lipschitz. At every step $t$, the learner $\A$ commits to an $x_t$ and the environment samples $f_t \sim \D$ which is then revealed to the learner. The aim of the learner $\A$ is to minimize regret defined as
\[ \mathrm{Regret}_{\mathrm{stoch}, \A} = \bbE[f_t(x_t)] - \min_{x \in \X} \bbE_{f \sim \D}[f(x)]\]


\begin{theorem}
\label{thm:hello}
hello
\end{theorem}
\begin{claim}
\label{claim:hello}
hello
\end{claim}
$\B, \bB, \bb, \bbE$
\pref{thm:hello}
\pref{claim:hello}



\section{An approach based on online gradient descent}

\def\x{\mathbf{x}}


\begin{algorithm}
	[H] \caption{noisy ogd} \label{alg:pogd}
	\begin{algorithmic}
		\FOR{$t=1$ to $T$}
		\STATE Play $\x_t$, observe loss $f_t(\x_t)$, and gradient $\nabla_t = \nabla f_t(\x_t)$.
		\STATE Let $n_t = N(0,\frac{1}{\eps} I )$
%		$$ \tilde{g}_t = N(\nabla_t , \frac{1}{\eps} I) $$ 
		\STATE Update
		%$$ \y_{t+1} \leftarrow \y_t - \eta_t \nabla_t  + n_t - n_{t-1}$$
		$$ \x_{t+1} = \prod_\K[\x_{t} - \eta (\nabla_t + n_t)]$$
		
		\ENDFOR
	\end{algorithmic}
\end{algorithm}


\begin{claim}
The algorithm above satisfies:
\begin{enumerate}
    \item 
    $$ \E[ \regret_T] \leq \frac{1}{\eps} DG \sqrt{T}  $$
    \item
    It is $\eps$ differentially private
\end{enumerate}
\end{claim}

Part 1 of the claim follows from lemma 6.3.1 in "introduction to online convex optimization". 

Part 2 I'm guessing should be true, for the same reason it is true in FPL: the ball (pre-projection) around $\x_t$ is of radius $\frac{1}{\eps}$. 

